Consensus on Demand

Digital money can be implemented efficiently by avoiding consensus. However, no-consensus implementations have drawbacks, as they cannot support smart contracts, and (even more fundamentally) they cannot deal with conflicting transactions. We present a novel protocol that combines the benefits of an asynchronous, broadcast-based digital currency, with the capacity to perform consensus. This is achieved by selectively performing consensus a posteriori, i.e., only when absolutely necessary. Our on-demand consensus comes at the price of restricting the Byzantine participants to be less than a one-fifth minority in the system, which is the optimal threshold. We formally prove the correctness of our system and present an open-source implementation, which inherits many features from the Ethereum ecosystem.

==> broadcastcoin.tex <==
\subsection{Algorithm}


%This algorithm thus shows how to implement a currency in the account model on top of a reliable broadcast primitive. We use the Double-Echo Broadcast by Bracha and Toueg \cite{bracha}.

The \bcoin algorithm implements Byzantine reliable broadcast (see \cref{algorithm:bcoin} in Appendix \ref{appendix:bcoin} for the complete pseudocode). 

\begin{definition}
\label{definition:rb}
Assuming that each honest server observes transactions from a set of conflicting transactions $\{t_0, t_1, . . . \}$, we say that a \textbf{Byzantine reliable broadcast} algorithm is secure if it satisfies the following properties:

\begin{enumerate}
    \item \textbf{Totality}: If some honest server accepts a transaction, every honest server will accept the same transaction. 
    \item \textbf{Agreement}: No two honest servers accept conflicting transactions. 
    \item \textbf{Validity}: If every honest server observes the same transaction (there are no conflicting transactions), this transaction is accepted by all honest servers. 
    \item \textbf{Honest-Termination}: If messages are delivered quickly and no conflicting transactions are present, the protocol terminates quickly.
\end{enumerate}
\end{definition}

To do so, the algorithm works in three steps. A transaction $t = (sender, sn, recipient, amount)$ undergoes the following steps before being safely executed:
\begin{enumerate}
    \item \textit{Dissemination}: A server broadcasts $t$ received by a client by sending it to all servers.
    \item \textit{Verification}: Servers acknowledge $t$ if they have never acknowledged a conflicting transaction $t'$. 
    \item \textit{Approval}: Servers that receive more than $\frac{n+f}{2}$ acknowledgements for a transaction, broadcast an {\tt APPROVE} message. Servers also broadcast an {\tt APPROVE} message, if they see more than $f+1$ approvals. A server that receives more than $2f + 1$ approvals, accepts the transaction and executes it as soon as all previous transactions are executed, and enough funds are available in the sender's balance.
\end{enumerate}

%Note that by only acknowledging transactions for which all transactions with lower sequence numbers have already been accepted, and where the sender is in possession of enough currency, we satisfy the additional property that if a transaction is accepted, then eventually every server will be able to execute it.
%This is opposed to transactions that might be seen as ``empty-promises'' until the sender actually obtains the necessary funds. 

% This property is a recurring topic..

We refer the reader to Appendix \ref{appendix:bcoin} for the proof of correctness of the presented algorithm.



\subsection{Correctness}

We show that \bcoin satisfies Byzantine reliable broadcast.

\textbf{Totality}: A server that accepts a transaction has seen $2f + 1$ {\tt APPROVE} messages. Out of these, at least $f+1$ come from honest servers. Since we use perfect links to propagate messages, eventually every honest server will receive these and broadcast their own {\tt APPROVE} message (line \ref{line:readywave}). Assuming $f < \frac{n}{5}$, eventually all $n-f > 2f + 1$ {\tt APPROVE} messages from honest servers will be received, and thus all honest servers will accept the transaction.

\textbf{Consistency}: Let us assume towards contradiction that server $u$ accepts $t$ and server $v$ accepts $t'$ for the same $(sender, sn)$ pair. Firstly, due to the no duplication property of the underlying perfect link, no Byzantine server can acknowledge the same transaction twice. Since $u$ and $v$ have both received a Byzantine quorum of more than $\frac{n+f}{2}$ acknowledgements, at least some honest server has acknowledged a transaction twice, which is a contradiction, as the \textit{ackedSN} array prevents this.

\textbf{Validity}: As all honest servers observe the same transaction, they all acknowledge it. Due to the underlying perfect link, acknowledgements are seen by every honest server, which will thus accept the transaction. 

\textbf{Honest-Termination}: As we do not require any input from Byzantine servers, if the messages from honest servers are delivered quickly, the protocol terminates quickly.


\subsection{Discussion}
\label{mapping:discussion}
Now that we have established the soundness of our scheme, this section discusses some details.
Most notably, contrary to the algorithm presented in \cite{MerelyBroadcastig}, we made the decision to not allow transactions to be broadcast before the required funds are available. Analogously, servers only acknowledge transactions once they see the funds required for it. 

This design makes sure that servers are guaranteed to eventually be able to execute confirmed transactions. 
%This is in contrast with transactions that can be seen as a potentially empty promise in Astro, as the required funds for a transaction might never be obtained by the transaction's sender.

This implies that only a single transaction can be in the unconfirmed state at any time. Otherwise, servers might be fooled into signing two consecutive transactions, where the first transaction might later turn out to be the “wrong" double-spend transaction. The actual accepted transaction might then not leave enough funds for the latter, leading to the server having acknowledged a transaction that could constitute an ``empty-promise'', nullifying the benefits mentioned above.

Next, we discuss alternatives to the broadcast scheme, more specifically addressing the number of messages used per transaction. The algorithm works in three rounds of communication: 

\begin{enumerate}
    \item The transaction is broadcast to all servers using $n$ messages. 
    \item Each of the $n$ servers then broadcasts their acknowledgment, requiring $n^2$ messages in total.
    \item Each of the $n$ servers broadcasts an approval message, either once enough acknowledgements or enough ready messages were received. This final step is required to guarantee totality and again requires $n^2$ messages. Note that trivially rebroadcasting the acknowledgements from step 2 would work as well if signatures were added, but instead would require $n^3$ messages.
\end{enumerate}

It is possible to improve the algorithm, such that only the recipient of a transaction collects acknowledgments, and later uses the acknowledgements as proof of reception of the transaction. This idea alleviates the need for step 3 entirely and improves message complexity to $\mathcal{O}(n)$.  
%The Astro II implementation published in \cite{MerelyBroadcastig} presents such an algorithm as well and explores the intricacies thereof. 
%It is left to future work to implement Consensus on Demand in this setting.




==> letter_to_reviewers.tex <==
\newpage
\section{Response Letter to First-Round Reviewers}

We thank the reviewers for their positive comments, appreciating the potential of our work and encouraging us to resubmit an improved write-up. Below we discuss the helpful feedback we received that guided further development and improvement of our paper.

We appreciate the reviewer's criticism of vague descriptions and confusing parts of our work, in particular the problem statement. Thus, we have reworked the problem statement section to clearly describe our objectives. While we reformulated the section to be more precise, we also aimed to keep the description as simple as possible in the interest of easy intuitive understanding, and we are hopeful that we have been able to improve the write-up in both respects.

We are thankful to the reviewers for directing our attention to the relevant work of Kuznetsov et al. \cite{kuznetsov2021revisiting}. Indeed, in the setting where the clients are a subset of servers our bound is improved to $n \geq 5f - 1$. We now reference this result and indicate its significance in the context of our work. We similarly appreciate the reviewers suggesting other papers to mention and compare our work to, which we now do.

According to the reviewers suggestions, we have now included more proofs in the main text, as well as simplified both the \bcoin and \apost algorithms, such that we could include the pseudocode in the main body. As requested, we removed many ambiguous and opinion-based statements, which the reviewers correctly pointed out. Similarly, we corrected the inconsistencies and confusing phrasing helpfully indicated by the reviewers.

Additionally, we included a discussion of the important questions raised by the reviewers, such as the potential for Byzantine clients to force the execution of the slow path. Due to the strict page limit we necessarily need to leave some topics related to our protocol outside the scope of this paper, but the reviewer's input helped us decide which related questions are most important to discuss, and we have edited the paper accordingly.

In the following, we briefly address each comment one by one.

\subsection{Review 1}

\begin{displayquote}
The consensus algorithm Multishot is not explained due to double blind policy (you could have uploaded an anonymised technical report).
\end{displayquote}
A quick description can now be found in \cref{implementation}, with the pseudocode and a proof sketch in \cref{appendix:multi}.

\begin{displayquote}
The identifier of a transaction in p.3 conflicts with the definition of a transaction at the end of p.6 since the latter contains a sender and receiver but not the former.
\end{displayquote}
We have made the definition of a transaction more precise on page 3. Additionally we removed the definition of a transaction identifier.

\begin{displayquote}
Table 1 lists HoneyBadger BFT, however, its randomized binary cconsensus [PODC'14] is known to suffer from a liveness issue. It would be better to compare against Red Belly Blockchain / DBFT that solves binary consensus deterministically [S\&P'21].
\end{displayquote}
We now compare our solution with Red Belly Blockchain, and use an algorithm from the BEAT family to display a fully asynchronous version of our algorithm. 

\begin{displayquote}
At times the terms 'no-consensus' is used, while at other times the term 'consensusless' is used. It should be made consistent.
\end{displayquote}
We have removed the term 'consensusless'.

\begin{displayquote}
Recent works [Kuznetsov et al., PODC 2021] showed that one can achieve a two message delay fast path consensus with partial synchrony when n>=5f-1. Why not using one of these partially consensus algorithms instead of a synchronous algorithm?
\end{displayquote}

\begin{displayquote}
The conclusion states that "no algorithm can tolerate a larger fraction of Byzantine servers while providing the optimal fast path" and cite [32]. Note, that this result was recently contradicted by the aforementioned paper at PODC'21.
\end{displayquote}
We present a fully asynchronous (and leaderless) algorithm. 
The work from Kuznetsov et al. is highly relevant, and in the special case where \textit{proposers} (clients) are a subset of \textit{acceptors}(servers) their insight can be applied to improve our resilience threshold from $n \geq 5f + 1$ to $n \geq 5f - 1$. In our model however, clients are external to servers and are free to enter and leave the system as they please. Under these assumptions, as Kuznetsov et al. admit n = 5f + 1 remains the optimal threshold.
\\\\
In light of this recent work, we have added the following to \cref{relatedwork}: 
\say{Kuznetsov et al. \cite{kuznetsov2021revisiting} have recently shown the lower bound to be $n \geq 5f - 1$ in the special case where the set of \textit{proposers} (clients) is a subset of \textit{acceptors} (servers). Their insight is to disregard the acknowledgement of a provably misbehaving server. Although we do not assume the required special case, as in our model the set of clients is external to servers and changing freely, the assumption might well be warranted in other contexts, wherein their approach is applicable to our work.}

\begin{displayquote}
Definition 3: "all by" -> "by all".
\end{displayquote}
We fixed this typo.

%\begin{displayquote}
%To conclude, I would recommend the authors to look at the recent work published at PODC’21 and correct their paper in the light of this new upper bound on the number of Byzantine failures to solve consensus in two message delays in the good case.
%\end{displayquote}
%Thank you!


\subsection{Review 2}

\begin{displayquote}
However, i feel that some concepts were not defined adequately.
\end{displayquote}
We have reworked the definitions and the problem statement.

\begin{displayquote}
Some of the pseudocode should be brought to the main body of the paper for better presentation.
\end{displayquote}
We have brought the pseudocode to the main body.

\begin{displayquote}
(...) it is not clear whether a byzantine client may force the system executing consensus repeatedly. What is the possibility for this to happen and can we do an analysis on the conditions that may prevent such attack?
\end{displayquote}
We have added a discussion of this problem.

\begin{displayquote}
Finally the increase on throughput is not justified by any means (e.g., by any experimental outcomes). It would be nice to at least have an extended discussion or analysis on the benefits on throughput.
\end{displayquote}
We now discuss the throughput results applicable to our protocol.

\begin{displayquote}
page 3: In definition 1 how are transactions compared (i.e. $t \neq t’$)?
\end{displayquote}
We have made this definition more clear.

\begin{displayquote}
page 3: Finality is not defined.
\end{displayquote}
We clarified the text.

\begin{displayquote}
page 7: in the operation bc.Balance what is v?
\end{displayquote}
We have changed the variable v to an amount $a$ of currency.

\begin{displayquote}
page 7: Definition of validity there is a small typo: “all by” => “by all”
\end{displayquote}
This typo was fixed.

\begin{displayquote}
page 8: it would be nice to have the pseudocode of the algorithm.
\end{displayquote}
The pseudocode was added.

\begin{displayquote}
page 9: same goes here a pseudocode will be helpful at least to show the decision to go for a consensus. Is one conflicting ack sufficient to trigger consensus?
\end{displayquote}
This pseudocode was added as well. We discuss this problem in \cref{discussion}.

\begin{displayquote}
page 10: typo in the Blocks paragraph: third line “instead” is a repetition
\end{displayquote}
We fixed this typo.

\begin{displayquote}
page 11: Figure 3 is not helpful. I find it hard to follow and the logic is unclear. I ‘d rather use the space for an algorithm instead.
\end{displayquote}
\cref{fig:implementation} was moved to the appendix.


\subsection{Review 3}

\begin{displayquote}
The authors do not define precisely the problem they solve.
\end{displayquote}
We have reworked the problem statement.

\begin{displayquote}
The authors describe their implementation, making sweeping claims like "Our
system achieves the unlimited throughput", "We propose a solution that... is
much closer to see real-world use". However, no experimental results are
provided to justify such claims.
\end{displayquote}
We have removed these opinionated claims. We now mention applicable experimental results in \cref{discussion}.


\begin{displayquote}
The presentation is inadequate, with algorithms explained poorly and major
decisions not justified.
\end{displayquote}
The presentation of our algorithms has been reworked.


\begin{displayquote}
Section 1: "But no-consensus payment systems also have a major weakness, as
they only have rudimentary means to deal with conflicting transactions." - You
need to put citations to explain which systems you're talking about.
\end{displayquote}
We have added citations and clarified the description of no-consensus payment systems.


\begin{displayquote}
Section 1: "We present a description that is very accessible" - this is in the
eye of the beholder.
\end{displayquote}
This claim was removed.

\begin{displayquote}
Section 2: "our goal in this work is to construct a more efficient consensus
protocol, defined as follows." - No, this isn't your goal. Your goal is to
construct a particular payment system, which you don't even define. You try to
sketch something at the end of Section 5.1, but really you have to give a formal
definition.

Definition 2: "If no conflicting transactions are present, the protocol
terminates in 1 communication round-trip." - why such a requirement? Is this why
you need 5f+1 replicas instead of 3f+1? If you want to demonstrate your ideas,
it could be simpler to go with the classical setting of 3f+1, even if it
requires more rounds.
\end{displayquote}
We have reworked and clarified the problem statement.


\begin{displayquote}
Def 3: What does "quickly" mean? This isn't a formal term.
\end{displayquote}
We have reformulated the problem statement, and fast termination is now no longer part of the definition of consensus.

\begin{displayquote}
Section 6: I found it difficult to follow this section, perhaps because the
formal framework is poorly defined (see above). The proof sketches should be in
the main text.
\end{displayquote}
This intuition section was reworked, and the proof sketches were added ot the main text.

\begin{displayquote}
Section 6.1: "for which they have received the most acknowledgements to the
consensus instance." - during which period of time?
\end{displayquote}
We have now clarified this: The most acknowledged transaction after having received $n-f$ acknowledgments is proposed to the consensus instance.

\begin{displayquote}
Section 3: "This requirement has been shown to be optimal by Martin et al.
[32]." - and then was shown to be not optimal by Kuznetsov et al., PODC'21.
\end{displayquote}
We now address the recent work by Kuznetsov et al. \cite{kuznetsov2021revisiting} in \cref{relatedwork}.

\begin{displayquote}
Fig 3: this isn't helpful. You'd better spend space defining your problem and
describing your solution more precisely.
\end{displayquote}
We have moved \cref{fig:implementation} to the appendix.

\begin{displayquote}
The paper requires proof-reading for English usage. There are lots of strange
sentences like "In 2016 Gupta [24] reminds the world", "do not need to rely on
comply broadcast primitives", etc.
\end{displayquote}
Phrasing was improved in these and other cases.



%\subsection{Detailed reviews}


%“Recent works [Kuznetsov et al., PODC 2021]”,
%“n>5f (...) there is room for improvement”,
%“The conclusion (...) contradicted by the aforementioned paper”,
%“I would recommend the authors to look at the recent work published at PODC’21”:

%We now cite and discuss Kuznetsov et al. \newline

%“The consensus algorithm Multishot is not explained(...)”:
%Did we change something? Can we just write “fixed”? xD

%“The identifier of a transaction in p.3 conflicts with the definition of a transaction”:
%Can we write something non-insulting here?

%“Table 1 lists HoneyBadger BFT (..) better to compare against Red Belly”:
%As suggested.

%“No-consensus, consensusless - should be made consistent.”:
%Fixed.

%“Definition 3”:
%Fixed.



%Review 2:

%“some concepts were not defined adequately”:
%Definitions are reworked.

%“some of the pseudocode should be brought to the main body”:
%As suggested.

%“it is not clear whether a byzantine client may force the system executing consensus”:
%We now discuss this problem.

%“the increase on throughput is not justified”:
%We now discuss the throughput results applicable to our protocol.

%“it would be nice to have the pseudocode of the algorithm”,
%“same goes here a pseudocode will be helpful”:
%As suggested.

%“In definition 1 how are transactions compared (i.e. $t \neq t’$)?”:
%Clarified.

%“Finality is not defined.”:
%No comment here?

%“in the operation bc.Balance what is v?”:
%This was rewritten? Do we say anything?

%“Definition of validity typo”,
%“typo in the Blocks paragraph”:
%Fixed.

%“Is one conflicting ack sufficient to trigger consensus?”:
%In general in complete asynchrony, sure it is. Do we say anything here?

%“Figure 3 is not helpful (...) rather use the space for an algorithm instead.”:
%As suggested.


%Review 3.

%“The authors do not define precisely the problem”:
%Problem statement is now reworked.

%“sweeping claims (...) no experimental results”:
%Removed opinions. We now mention applicable experimental results.

%“presentation is inadequate, with algorithms explained poorly and major
%decisions not justified”:
%Algorithm presentation is now reworked.

%Detailed comments:

%“put citations to explain which systems”:
%Now cited, clarified.

%“this is in the eye of the beholder”:
%Removed opinions.

%“Your goal (...) you don't even define.”,
%%“Definition 2: (...) - why such a requirement?”,
%“What does "quickly" mean?”:
%Problem statement is now reworked and clarified.

%“The proof sketches should be in the main text.”:
%As suggested

%“for which they have received the most acknowledgements (...)" - during which period of time?”:
%Now clarified.
%
%“shown to be not optimal by Kuznetsov et al., PODC'21.”:
%We now cite and discuss Kuznetsov et al.

%“Fig 3: this isn't helpful. You'd better spend space defining your problem and
%describing your solution more precisely.”:
%As suggested.

%“English usage (..) strange sentences”:
%Improved.





%First and foremost we believe that we have laid out our goals with improved formalism in the problem statement section.

%We have simplified both the \bcoin and \apost algorithms, such that we could include the pseudocode in the main body, as was requested in your reviews. Instead of relying of on our own flavor of reliable broadcast, we abstract this complexity away. We believe that this puts more focus on the more important contributions.

%Towards the same goal of improved readability, we have changed the intuition section to be more precise and concise.

%As another major improvement, we have included a more thorough discussion on why this proposed digital currency is equally or more scalable than current state of the art. In this section, we also address a remark from reviewer 2, on whether Byzantine clients can force the execution of the slow path.

%We are thankful to the two reviewers who pointed us to recent relevant work by Kuznetsov et al. \cite{kuznetsov2021revisiting} at PODC 2021. This improvement wasn't known to us previously, and we have adapted the related work section accordingly and mention the subtle improvement in the discussion as well. Sadly, we believe that it does not apply to the case of digital currencies that we present here, as the set of clients is almost never a subset of the set of servers. Indeed, Kuznetsov et al. mention in section 4.4, that n = 5f + 1 remains the optimal threshold in that case (our clients are proposers and Leslie Lamport's model and servers take the role of acceptors). Another key difference lies in the model, as we do not rely on leader election and therefore do not need to assume partial synchrony for our presented algorithm.

%We have added DBFT / Red Belly Blockchain in our comparison table, as we agree that it makes for an interesting comparison. The reason we have chosen Honey Badger BFT / BEAT to be paired with \apost was simply to portray how no synchrony assumptions are required.

%Finally, we believe that we have addressed all typos that you rightfully pointed out. We have removed Figure 3 (that was showing implementation details) as it was perceived as distracting, and have tidied up the definition of a transaction and a payment system in general.


==> lowerbounds.tex <==

\section{Impossibility results}

\begin{theorem}
A system with $n$ servers cannot reach consensus with a fast path of 1 communication round with $f \geq \frac{n}{5}$ in the asynchronous model.
\end{theorem}

\begin{proof}
We assume towards contradiction that there exists an algorithm that reaches consensus for $n$ servers with $f \geq {\frac{n}{5}}$, while having a fast path of just 1 communication round.

Let us divide the $n$ servers into three groups. Two groups of size $n-2f$ and $f$ respectively contain only honest servers while a third group of size $f$ contains all byzantine servers.
Let the larger group of honest servers acknowledge the transaction $t$, while the smaller group acknowledges $t'$. The group of byzantine servers can acknowledge either transaction. 

Due to scheduling a server $s$ might see $(n-2f) + f = n-f$ support messages for a transaction $t$. The server $s$ might not receive any more messages, and in order to satisfy termination through the fast path as well as validity, $s$ must decide on $t$.

On the other hand, for all other servers the adversary can delay up to $f$ acknowledgements for $t$, i.e., all other servers will only observe $n-3f$ messages acknowledging $t$. Since $2f \geq n-3f$, the adversary can guarantee that every other server observes at least as many acknowledgements for $t'$ as for $t$. Eventually the remaining servers will have to decide on either transaction in order to satisfy termination. Servers might very well decide on $t'$, which violates the agreement property.
\end{proof}

\begin{theorem}
A system with $n$ servers cannot reach consensus with a fast path of 1 round of communication with $f \geq \frac{n}{4}$ in the synchronous model. 
\end{theorem}

\begin{proof}
We assume towards contradiction that there exists an algorithm that reaches consensus for $n$ servers with $f \geq {\frac{n}{4}}$, while having a fast path of a single communication round.

Again, let us divide the $n$ servers into three groups. Two groups of size $n-2f$ and $f$ respectively contain only honest servers while a third group of size $f$ contains all byzantine servers.
Let the larger group of honest servers acknowledge the transaction $t$, while the smaller group acknowledges $t'$. The group of byzantine servers can acknowledge either transaction. 

A server $s$ might see $(n-2f) + f = n-f$ acknowledgements for a transaction $t$ and just $f$ acknowledgments for $t'$. In order to satisfy termination through the fast path as well as validity, $s$ must decide on $t$.

Since $2f \geq n-2f$, the adversary can make sure that all other servers observe at least as many acknowledgements for $t'$ as for $t$. The remaining servers will eventually have to decide on either transaction in order to satisfy termination. Servers might very well decide on $t'$, which violates the agreement property.

\end{proof}
